Constant-Rate Certified Deletion

We present a unified framework for upgrading a broad class of cryptographic primitives to support constant-rate certified deletion. Previous constructions require a linear number of qubits per encrypted bit of certified-deletable plaintext. In contrast, we obtain the first constant-rate constructions in the plain model that achieve certified deletion while preserving everlasting security. Our approach applies to a wide range of "all-or-nothing"-type primitives based on BB84-style encodings, including commitment schemes, public-key encryption, attribute-based encryption, and fully homomorphic encryption. Beyond this class, we also obtain constant-rate certified deletion for primitives built from subspace coset states, such as blind delegation, secure software leasing, functional encryption, and differing-inputs iO, and CCA-PKE. Importantly, our framework does not introduce any additional assumptions beyond those required by the underlying certified deletion primitives. Finally, under the hardness of SIS, we show that public verifiability can be incorporated into BB84- and coset-based certified deletion. In combination with our constant-rate constructions, this yields publicly verifiable certified deletion schemes with constant rate.

==> 6-1_coset_states.tex <==
\ifnum\llncs=0
\section{Certified Deletion for Subspace Coset States}\label{section:coset_m}
\fi
\ifnum\llncs=1
\section{Omitted Details from Section~\ref{section:coset_m}.}
\fi

% Tilde looks strange
\subsection{Main Theorem}\label{section:coset}

We define the notion of subspace hiding, which is similar to $\cite{BGK+}$. However, we additionally require a string to be hidden semantically.
\begin{definition}[Subspace Hiding]\label[definition]{subspace_hiding}
    Let $\mathscr{A}$ be a class of adversaries.\footnote{As \cite{BGK+} mentioned, $\mathscr{A}$ should be closed under constant-factor increases in space and time.} We say that a QPT operation $\{\cZ_\lambda\}_{\lambda \in \N}$ is \textbf{subspace-hiding} for $\mathscr{A}$ if there exists a QPT simulator $\{\cS_\lambda\}_{\lambda \in \N}$ such that for any adversary in $\mathscr{A}$, the advantage in the following game is negligible in $\lambda$:
    \begin{enumerate}
        \item Let $n=4\lambda$. Sample $[S,T]$ uniformly at random over dimension $n$. Also, sample $(u,w) \leftarrow \co(T) \times \co(S^\perp)$ and a string $r \in \F^k$. Then they send these variables to the challenger.
        \item The challenger samples $G$, a uniformly random superspace of $S^\perp$ of dimension $\frac{3n}{4}$. Let $x \in \co(G)$ be the unique coset such that $S^\perp + w \subset G +x$. Next, the challenger samples two challenges $c_a,c_b \leftarrow \{0,1\}$. If $c_a=0$, they compute $\cZ_\lambda(S,T,u,w,r)$. If $c_a=1$, they compute $\cZ_\lambda(S,T,u,w,0)$. If $c_b=0$, they compute $\cZ_\lambda(S,T,u,w,0)$. If $c_b=1$, they compute $\cS_\lambda(G,T,u,x,0)$. Then, they send two outputs to the adversary.
        \item The adversary output two guesses $c_a',c_b' \in \{0,1\}$ for $c_a$ and $c_b$.
    \end{enumerate}
    The adversary's advantage is defined to be $\max\left\{\left|\Pr[c_a'=c_a]-\frac{1}{2} \right|, \left|\Pr[c_b'=c_b]-\frac{1}{2} \right| \right\}$.
\end{definition}

Before presenting the main theorem, we illustrate the relationships among the different subspaces and vectors in the following figure. Each blue rectangle represents a vector space. An overlap between the sides of two rectangles indicates that they share a subset of basis vectors, with the size of the overlap corresponding to the dimension of the shared subspace.


\begin{figure}[!t]
\centering
\resizebox{0.98\linewidth}{!}{%
\begin{tikzpicture}[
  line/.style={blue!80!black, very thick},
  note/.style={red, font=\normalsize},
  lab/.style={blue!80!black, font=\normalsize},
  top/.style={green!70!black, font=\normalsize},
  every node/.style={font=\normalsize}
]

% ============================================================
% Left diagram
% ============================================================
\begin{scope}[shift={(0,0)}]

% geometry
\def\W{6}
\def\H{3}
\def\xhalf{3.0}       % 1/2
\def\xfive{3.75}      % 5/8
\def\xthree{4.5}      % 3/4
\def\xlabelshift{3.56} % slightly left of 5/8

% top green labels
\node[top] at (-1.9,3.35) {$\dim$};
\node[top] at (-0.2,3.35) {$0$};
\node[top] at (\xhalf,3.35) {$\frac{n}{2}$};

% outer rectangle
\draw[line] (0,0) rectangle (\W,\H);

% horizontal lines
\draw[line] (0,2.1) -- (\W,2.1);
\draw[line] (0,1.25) -- (\W,1.25);

% vertical lines
\draw[line] (\xhalf,2.1) -- (\xhalf,\H);      % top row
\draw[line] (\xfive,1.25) -- (\xfive,2.1);   % second row
\draw[line] (\xthree,0) -- (\xthree,1.25);   % bottom row

% labels
\node[lab] at (1.5,2.55) {$S$};
\node[lab] at (4.5,2.55) {$\mathrm{co}(S)$};

\node[lab] at (1.5,1.68) {$S^{+}$};

\node[lab] at (2.25,0.6) {$T$};
\node[lab] at (5.25,0.6) {$\mathrm{co}(T)$};

% red annotations
\node[note] at (3.36,1.68) {$v_{0c}$};
\node[note] at (4.12,1.68) {$v_{0d}$};
\node[note] at (5.25,1.68) {$u$};

% red curves
% v_{0c}: from 1/2 to 5/8
\draw[red, thick]
  (3.03,1.25) .. controls (3.18,1.48) and (3.57,1.48) .. (3.72,1.25);

% v_{0d}: from 5/8 to 3/4
\draw[red, thick]
  (3.78,1.25) .. controls (3.92,1.48) and (4.33,1.48) .. (4.47,1.25);

% u: from 3/4 to right end
\draw[red, thick]
  (4.53,1.25) .. controls (4.85,1.48) and (5.68,1.48) .. (5.97,1.25);

% green label under second row, shifted slightly left
\node[top] at (\xlabelshift,0.98) {$\frac{3n}{4}-k+1$};

% blue curve for A: endpoints attached to bottom edge
\draw[blue!80!black, thick]
  (\xhalf,0) .. controls (3.25,-0.38) and (4.25,-0.38) .. (\xthree,0);

\node[lab] at (3.75,-0.52) {$A$};
\node[top] at (\xthree,-0.55) {$\frac{3n}{4}$};

% bottom formula: red, with A in blue
\node[note] at (\W/2,-1.55)
  {$v_0 \coloneqq v_{0c}+v_{0d} \in {\color{blue!80!black}A}$};

\end{scope}

% ============================================================
% Right diagram
% ============================================================
\begin{scope}[shift={(10.9,0)}]

% geometry
\def\W{6}
\def\H{3}
\def\xhalf{3.0}       % 1/2
\def\xfive{3.75}      % 5/8
\def\xthree{4.5}      % 3/4
\def\xlabelshift{3.56} % slightly left of 5/8

% top green labels
\node[top] at (\xhalf,3.35) {$\frac{n}{2}$};
\node[top] at (5.65,3.35) {$0$};
\node[top] at (6.75,3.35) {$\dim$};

% outer rectangle
\draw[line] (0,0) rectangle (\W,\H);

% horizontal lines
\draw[line] (0,2.1) -- (\W,2.1);
\draw[line] (0,1.25) -- (\W,1.25);

% vertical lines
\draw[line] (\xhalf,2.1) -- (\xhalf,\H);      % top row
\draw[line] (\xfive,1.25) -- (\xfive,2.1);   % second row
\draw[line] (\xthree,0) -- (\xthree,1.25);   % bottom row

% labels
\node[lab] at (1.5,2.55) {$\mathrm{co}(S^\perp)$};
\node[lab] at (4.5,2.55) {$S^\perp$};

\node[lab] at (5.25,1.68) {$(S^{+})^\perp$};

\node[lab] at (2.25,0.6) {$\mathrm{co}(T^\perp)$};
\node[lab] at (5.25,0.6) {$T^\perp$};

% red annotations
\node[note] at (1.5,1.68) {$w$};
\node[note] at (3.36,1.68) {$\tilde v_{0c}$};
\node[note] at (4.12,1.68) {$\tilde v_{0d}$};

% red curves
% w: below the lower edge of co(S^\perp), concave downward
\draw[red, thick]
  (0.03,2.10) .. controls (0.65,1.86) and (2.35,1.86) .. (2.97,2.10);

% \tilde v_{0c}: from 1/2 to 5/8
\draw[red, thick]
  (3.03,1.25) .. controls (3.18,1.48) and (3.57,1.48) .. (3.72,1.25);

% \tilde v_{0d}: from 5/8 to 3/4
\draw[red, thick]
  (3.78,1.25) .. controls (3.92,1.48) and (4.33,1.48) .. (4.47,1.25);

% green label under second row, shifted slightly left
\node[top] at (\xlabelshift,0.98) {$\frac{n}{4}+k-1$};

% blue curve for B: endpoints attached to bottom edge
\draw[blue!80!black, thick]
  (\xhalf,0) .. controls (3.25,-0.38) and (4.25,-0.38) .. (\xthree,0);

\node[lab] at (3.75,-0.52) {$B$};
\node[top] at (\xthree,-0.55) {$\frac{n}{4}$};

% bottom formula: red, with B in blue
\node[note] at (\W/2,-1.55)
  {$\tilde v_0 \coloneqq \tilde v_{0c}+\tilde v_{0d} \in {\color{blue!80!black}B}$};

\end{scope}

\end{tikzpicture}%
}
\caption{Coset basis decomposition.}
\label{fig:coset-basis}
\end{figure}




\begin{theorem}\label[theorem]{coset_maintheorem}
    Let $\lambda$ be the security parameter. Fix $k,n \in \N$ such that $8k+\Theta(\lambda) \leq n$. Consider a family of finite prime fields $\{\F_\lambda\}_\lambda$ with polynomial bounded field sizes. Let $\regR \in \F^{k \times n}$ be a matrix that is both MDS and satisfies Row-Resilient Column Independence (\cref{prop_extract}).
    Let $m \in \F^k$ be classical messages and $\{\Zs_\lambda(\cdot)\}_{\lambda \in \N}$ be a quantum operation with classical input. Define the following distribution $\left\{\EXP_\lambda^{\As_\lambda}(m) \right\}_{\lambda \in \N }$ over quantum states, obtained by running $\As_\lambda$ as follows.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage (Definition~\ref{sampling}).
        
        Next, sample $(v,w) \leftarrow \co(S) \times \co(S^\perp)$, uniformly at random. Let $u \in \co(T)$ be the unique coset such that $S+v \subset T+u$. 
        
        Finally, sample a uniform random string $r \in \F^n$.
        Initialize $\As_\lambda$ with
        \begin{equation*}
            \ket{S_{v,w}}, m+\regR \regB^{-1} v+r, \Zs_\lambda(S, T, u, w, r). 
        \end{equation*}
        \item $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^n$ and a residual state $\rho$. If $\widetilde{z} \in S^\perp + w$, then output $\rho$, and otherwise output a special symbol $\bot$.
    \end{enumerate}
    Let $\mathscr{A}$ be a class of adversaries that contains QPT algorithms. If $\{\cZ_\lambda\}_{\lambda \in \N}$ is subspace-hiding for $\mathscr{A}$ (\cref{subspace_hiding}), then for all $\{\cA_\lambda\}_{\lambda \in \N} \in \mathscr{A}$ and for all $m \in \F^k$,
    \begin{equation*}
        \TD\left(\EXP_\lambda^{\As_\lambda}(m), \EXP_\lambda^{\As_\lambda}(0^k) \right) = \negl(\lambda).
    \end{equation*}
\end{theorem}

\begin{proof}[Proof of \cref{coset_maintheorem}]
    We W.L.O.G. assume the row-resilient column independence properties holds for columns between $\frac{3n}{4}-k+2$ to $\frac{3n}{4}$. 
    
    To prove the theorem, we define a sequence of hybrid distributions.
    We start by defining $\hyb_0(m)$ to be identical to $\EXP_\lambda^{\As_\lambda}(m)$. Our goal is therefore to show that $\hyb_0(m)$ and $\hyb_0(0^k)$ are statistically close for all $m$.
    We establish this via a hybrid argument over individual field elements. Without loss of generality, we focus on the first coordinate: specifically, we show that $\hyb_0(m)$ and $\hyb_0(m+\alpha e_1)$ are statistically close for any $\alpha \in \F$, where $e_1 = 1|0^{k-1}$.
    To this end, we introduce a sequence of hybrid experiments from $\hyb_0$ to $\hyb_4$, such that each pair of consecutive hybrids is statistically indistinguishable. It therefore suffices to show that $\hyb_4(m)$ and $\hyb_4(m+\alpha e_1)$ are statistically close. This final step relies on the extraction lemma from \cref{coset_extractor}.
    Applying the extraction lemma requires that the challenger’s quantum state satisfies a specific structural condition. This condition is enforced by inserting a measurement $\mathcal{M}$ in $\hyb_4$. To argue that introducing $\mathcal{M}$ only negligibly affects the experiment, we show that its outcome is almost fixed and invoke the gentle measurement lemma.
    To establish this, we further introduce sub-hybrids $\hyb_2^a$ through $\hyb_2^f$. The consecutive games are  indistinguishable by the subspace-hiding security of $\cZ$, and if the outcome distribution of $\mathcal{M}$ were to change noticeably, the measurement result itself would yield a predicate that distinguishes the hybrids, since the measurement can be efficiently implemented.
    
    \paragraph{$\hyb_0(m)$:} This is the distribution $\{\EXP_\lambda^{\As_\lambda}(m)\}_{\lambda \in \N}$ described above.

    \paragraph{$\hyb_1(m)$:} In this hybrid, the first field element of the second register (which contains information about the message) is replaced by a uniformly random field element $b \leftarrow \F$. The dependence on the message $m$ is deferred until after the adversary sends a proof $\widetilde{z}$.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(v,w) \leftarrow \co(S) \times \co(S^\perp)$, \textcolor{red}{a field $b \leftarrow \F$}, and a string $r \leftarrow \F^k$. Let $u \in \co(T)$ be the unique coset such that $S+v \subset T+u$. Prepare
        \begin{equation*}
            \ket{S_{v,w}}_{A_1}
        \end{equation*}
        \item Initialize $\As_\lambda$ with
        \begin{equation*}
            A_1, \ \textcolor{red}{b}\|(m+\regR \regB^{-1} v+r)[2:k], \ \Zs(S, T, u, w, r).
        \end{equation*}$
        \As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$ and a residual state $\rho$.
        \item If \textcolor{red}{$b \neq (m+\regR\regB^{-1} v+r)[1]$} or $\widetilde{z} \not\in S^\perp + w$, then output $\bot$. Otherwise, output $\rho$.
    \end{enumerate}

    \paragraph{$\hyb_2(m)$:} In this hybrid, $\ket{S_{v,w}}_{A_1}$  is obtained by purifying the choice of $v$, followed by a measurement.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. \textcolor{red}{Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$}, a field $b \leftarrow \F$, and a string $r \leftarrow \F^k$. Prepare
        \begin{equation*}
            \frac{1}{\sqrt{|A|}} \sum_{v_0 \in A}\ket{v_0}_{C_1}\ket{S_{v_0+u,w}}_{A_1},
        \end{equation*}
        where $A = \co(S) \cap T$. \textcolor{red}{Measure the $C_1$ register and obtain $v_0$}. Let $v=v_0+u$.
        \item Initialize $\As_\lambda$ with
        \begin{equation*}
            A_1, \ b\|(m+\regR \regB^{-1} v+r)[2:], \ \Zs(S, T, u, w, r).
        \end{equation*}
        $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$ and a residual state $\rho$.
        \item If $b \neq (m+\regR\regB^{-1} v+r)[1]$ or $\widetilde{z} \not\in S^\perp + w$, then output $\bot$. Otherwise, output $\rho$.
    \end{enumerate}

    \paragraph{$\hyb_3(m)$:} In this hybrid, $v_0$ is purified, and its choice is deferred until after the adversary sends a proof $\widetilde{z}$.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and a string $r \leftarrow \F^k$. {\color{red} Prepare}
        \begin{align*}
            \frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} \ &\ket{v_0}_{C_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{C_2} 
            \otimes \\
            &\ket{S_{v_0+u,w}}_{A_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{A_2},
        \end{align*}
        where $A = \co(S) \cap T$.
        \item  Initialize $\As_\lambda$ with
        $A_1A_2$ and $\Zs(S, T, u, w, r)$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$ and a residual state $\rho$.
        \item \textcolor{red}{Measure the $C_1$ register and obtain $v_0$. Let $v=v_0+u$.} If $b \neq (m+\regR\regB^{-1} v+r)[1]$ or $\widetilde{z} \not\in S^\perp + w$ then output $\bot$. Otherwise, output $\rho$.
    \end{enumerate}

    \paragraph{$\hyb_4(m)$:} In this hybrid, we insert a projective measurement immediately before Step 3 of the previous hybrid $\hyb_3(m)$. We define the measurement $\cM$ immediately after describing the hybrid.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and a string $r \leftarrow \F^k$. Prepare
        \begin{align*}
            \frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} \ &\ket{v_0}_{C_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{C_2} \otimes  
             \\
            &\ket{S_{v_0+u,w}}_{A_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{A_2},
        \end{align*}
        where $A = \co(S) \cap T$. 
        \item Initialize $\As_\lambda$ with
        $A_1A_2$ and $\Zs(S, T, u, w, r)$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$ and a residual state $\rho$.
        \item \textcolor{red}{Apply a projective measurement $\{\Ms, I-\Ms\}$ and post-selecting on obtaining the outcome $I-\Ms$.}
        \item Measure the $C_1$ register and obtain $v_0$. Let $v=v_0+u$. If $b \neq (m+\regR\regB^{-1} v+r)[1]$ or $\widetilde{z} \not\in S^\perp + w$, then output $\bot$. Otherwise, output $\rho$.
    \end{enumerate}

    \paragraph{Definition of projective measurement $\{\cM,I-\cM\}$:} 

    We will define a CPTP map $\Phi$, and let $Q$ be a unitary that uses extra ancilla and defers all measurements in $\Phi$. The projective measurement $\cM$ is then defined as $Q^\dagger \Pi Q$, where $\Pi:=\ket{0}\bra{0}_{\text{Ans}}$ denotes the orthogonal projector. $\Phi$ is defined as follows:
    \begin{enumerate}
        \item Measure $C_{2}$ in computational basis and obtain $b\|\ell$.
        \item Apply $U$ on register $C_1$, where $U$ is defined in \cref{coset_unitaryconstruct}. Measure $C_{1}$ in computational basis and obtain $\widetilde{v}_0$. Parse $\widetilde{v}_0 := \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in \left(S^+\right)^\perp / T^\perp$.
        \item If $\widetilde{z} \not\in S^\perp + w$ or $\widetilde{z} \in \left(S^+\right)^\perp + \widetilde{v}_{0c}+w$, then set the ``Ans'' register as $\ket{1}$. Otherwise, set it as $\ket{0}$.
    \end{enumerate}
    

% Analyzing Hybrids=================================================================
\paragraph{Analyzing the Hybrids.} 
In the following, we relate $\TD(\hyb_{i}(m),\hyb_{i}(m+\alpha e_1))$ for different $i $.

\begin{lemma}\label[lemma]{coset_mainhybrid_0to3}
    Let $e_1 \in \F^k$ be the indicator string in which all positions are 0 except the first position, which is 1. For all $m \in \F^k$ and for all $\alpha \in \F$, we have
    \begin{align*}
        &\ \frac{1}{|\F|} \cdot \TD\left(\hyb_0(m), \hyb_0(m + \alpha\cdot e_1) \right) \\
        = &\ \TD\left(\hyb_1(m), \hyb_1(m + \alpha\cdot e_1)  \right) \\
        = &\ \TD\left(\hyb_2(m), \hyb_2(m + \alpha\cdot e_1)  \right) \\
        = &\ \TD\left(\hyb_3(m), \hyb_3(m + \alpha\cdot e_1)  \right).
    \end{align*}
\end{lemma}

\begin{proof}
    The first equation follows from the same argument as in \cref{bb84_mainhybrid_0to2} of the BB84-based protocol.
    Next, consider the second equation. We know that $\co(S) = A \oplus \co(T)$. In $\hyb_1$, a vector $v$ is sampled uniformly from $\co(S)$, which is equivalent to sampling $v_0$ uniformly from $A$ and $u$ uniformly from $\co(T)$ in $\hyb_2$, and then setting $v=v_0+u$.

     Finally, consider the third equation. We simply defer the measurement of $C_1$ until after the adversary outputs. This deferring process does not change the distribution, since the adversary's operation commutes with the operation on $C_1$. 
\end{proof}


For relating the trace distance in $\hyb_3$ and that in $\hyb_4$, we need the following lemma. Since the proof is somewhat involved, we defer the proof for the time being.
\begin{lemma}\label{lem:coset-predicate}
    For all $m \in \F^k$, the measurement outcome at Step 3 in $\hyb_4(m)$ yields the outcome $I-\Ms$ with $1-\negl(\lambda)$ probability.
\end{lemma}

The following Lemma follows from \cref{lem:coset-predicate} and is similar to \cref{bb84_mainhybrid_2to3}; hence, we omit the proof.
\begin{lemma}\label[lemma]{coset_mainhybrid_3to4}
    For all $m \in \F^k$ and $\alpha \in \F$, we have
    \begin{equation*}
        \TD\left(\hyb_3(m), \hyb_3(m + \alpha\cdot e_1)  \right) 
        \leq  \TD\left(\hyb_4(m), \hyb_4(m + \alpha\cdot e_1)  \right) +\negl(\lambda).
    \end{equation*}
\end{lemma} 



\begin{lemma}\label[lemma]{coset_mainhybrid4}
    For all $m \in \F^k$ and $\alpha \in \F$, we have
    \begin{equation*}
        \TD\left(\hyb_4(m), \hyb_4(m + \alpha\cdot e_1) \right) \leq \negl(\lambda).
    \end{equation*}
\end{lemma}

\begin{proof}
    First three steps of $\hyb_4$ are independent of $m[1]$. Hence, the challenger's and the adversary's joint view after Step 3 is identical between $\hyb_4(m)$ and $\hyb_4(m + \alpha\cdot e_1)$. 
        
    The measurement outcome $I-\cM$ guaranties that if we apply $U$ on $C_1$ register and measure the register to obtain $\widetilde{v}_0$. Then the following holds: Parse $\widetilde{v}_0 := \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in \left(S^+\right)^\perp / T^\perp$. Either (a) $\widetilde{z} \in S^\perp + w$ or (b) $\widetilde{z} \in (S^+)^\perp + \widetilde{v}_{0c} + w$.

    Suppose we condition on the case where event (b) does not occur. Then, there is no advantage between the two hybrids, since the hybrids always output $\bot$ in step 4. Moreover, event (b) does not occur with the same probability in both hybrids. Therefore, it suffices to condition on the case where event (b) occurs. Moreover, even under this condition, the joint view of the challenger and the adversary remains identical between $\hyb_4(m)$ and $\hyb_4(m + \alpha\cdot e_1)$. 

    We know that $\widetilde{v}_0 \in B$ by the same proof in Claim~\ref{coset_applyU}. Also, if the event (b) occurs $\widetilde{v}_{0c}$ must be a unique vector such that $\widetilde{z}-\widetilde{v}_{0c}-w \in (S^+)^\perp$. Hence, the state after step 3 must have the form
    \begin{equation*}
        \frac{1}{\sqrt{|\F|^{k-1}}}\sum_{h \in \left(S^{+}\right)^\perp / T^\perp } U^\dagger \ket{\widetilde{v}_{0c}+h}_{C_1} \otimes \ket{\psi_h}_{\cA},
    \end{equation*}
    %\synote{$S^{+}$ instead of $S^{\ell'}$?}
    where $\ket{\psi_h}$ is a normalized state that may be arbitrary entangled with register $C_1$ and $\widetilde{v}_{0c}$ is the unique vector defined by $\widetilde{z}$. Moreover, $\{\psi_h\}_h$ remains identical between $\hyb_4(m)$ and $\hyb_4(m +\alpha\cdot e_1)$.
        
    By the extractor \cref{coset_extractor}, we know that if we measure $C_1$ register and obtain $v_0$, then $\regR\regB^{-1}(v_0+u)$ is uniformly random and independent to adversary's view. Hence, checking whether $b \neq (m+\regR\regB^{-1} v+r)[1]$ or $b \neq (m+\regR\regB^{-1} v+r)[1]+\alpha$ occurs with equal probability and is independent of the residual state $\rho$. Note that although $r$ is sampled uniformly at random, it is not independent of the adversary's view and therefore is not a good source of randomness.
    \end{proof}

    \paragraph{Putting everything together, we conclude the proof of \cref{coset_maintheorem}.} By \cref{coset_mainhybrid_0to3,coset_mainhybrid_3to4,coset_mainhybrid4},
    \begin{align*}
        \TD(\hyb_0(m),\hyb_0(0)) &\leq \sum_{i=1}^{k} \TD\left(\hyb_0\left(0^{i-1} \| m[i:k]\right),\hyb_0\left(0^{i} \| m[i+1:k]\right)\right) \\
        &\leq k \cdot |\F| \cdot \negl(\lambda) \\
        &= \negl'(\lambda),
    \end{align*}
    where the first inequality follows from the triangle inequality and the second inequality follows from \cref{coset_mainhybrid_0to3,coset_mainhybrid_3to4,coset_mainhybrid4}. Note that previous hybrids and Claims  are all based on ``guessing'' the first bit as $b$. We need to slightly modified all the hybrids and Claims for each $i$. For example, in $\hyb_1$, we have to replace the $i$th bit of $\left(m+\regR\regB^{-1}v+r\right)$ with $b$ at Step 2. Also, check whether $b \neq \left(m+\regR\regB^{-1}v+r\right)[i]$ at Step 3. The modification is straightforward and we omit the details.
\end{proof}



    
    %===============================================================================================

    It remains to prove Lemma~\ref{lem:coset-predicate}, which claims that the measurement result is $I-\cM$ in $\hyb_4$ with overwhelming probability. The rest of this subsection is devoted to the proof of the lemma.

\begin{proof}[Proof of Lemma~\ref{lem:coset-predicate}]
    We introduce the following ``branch-hybrids'', $\hyb_3^a(m)$ through $\hyb_3^f(m)$, to argue that the projective measurement $\{\mathcal{M}, I-\mathcal{M}\}$ inserted in $\hyb_3(m)$ yields the outcome $I-\mathcal{M}$ with overwhelming probability, under the subspace-hiding security of $\mathcal{Z}(\cdot)$.
    
    \paragraph{$\hyb_3^a(m)$:} This is the same as $\hyb_4(m)$, except that $\hyb_3^a(m)$ does not defer the measurement and does not perform post-selection. Moreover, the experiment stops after the measurement outcome $I-\mathcal{M}$ or $\mathcal{M}$ is obtained.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and a string $r \leftarrow \F^k$. Prepare
        \begin{align*}
            \frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} \ &\ket{v_0}_{C_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{C_2} 
            \otimes \\
            &\ket{S_{v_0+u,w}}_{A_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{A_2},
        \end{align*}
        where $A = \co(S) \cap T$.
        \item Initialize $\As_\lambda$ with
        $A_1A_2$ and $\Zs(S, T, u, w, r)$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$.
        \item Measure $C_2$ in computational basis and obtain $b\|\ell$.
        \item Apply $U$ on register $C_1$. Measure $C_1$ and obtain $\widetilde{v}_0$. Parse $\widetilde{v}_0 := \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in \left(S^+\right)^\perp / T^\perp$.
        \item If $\widetilde{z} \not\in S^\perp + w$ or $\widetilde{z} \in \left(S^+\right)^\perp + \widetilde{v}_{0c}+w$, then return $I-\cM$. Otherwise, output $\cM$.
    \end{enumerate}

    \paragraph{$\hyb_3^b(m)$:} In this hybrid, the operation of measuring $C_2$ is moved to occur before the initialization of $\cA_\lambda$’s register. In addition, $\Zs(S, T, u, w, r)$ is replaced by $\Zs(S, T, u, w, 0^k)$.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and a string $r \leftarrow \F^k$. Prepare
        \begin{align*}
            \frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} \ &\ket{v_0}_{C_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{C_2} 
            \otimes \\
            &\ket{S_{v_0+u,w}}_{A_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{A_2},
        \end{align*}
        where $A = \co(S) \cap T$.
        \item \textcolor{red}{Measure $C_2$ in computational basis and obtain $b\|\ell$.}
        \item Initialize $\As_\lambda$ with
        $A_1A_2$ and $\Zs(S, T, u, w, \textcolor{red}{0^k})$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$.
        \item Apply $U$ on register $C_1$. Measure $C_1$ and obtain $\widetilde{v}_0$. Parse $\widetilde{v}_0 := \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in \left(S^+\right)^\perp / T^\perp$.
        \item If $\widetilde{z} \not\in S^\perp + w$ or $\widetilde{z} \in \left(S^+\right)^\perp + \widetilde{v}_{0c}+w$, then return $I-\cM$. Otherwise, output $\cM$.
    \end{enumerate}

    \paragraph{$\hyb_3^c$:} In this hybrid, the register $A_2$ is unentangled from the other registers. Also, we explicitly specify the construction of the register $C_2$.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and \textcolor{red}{a leakage $\ell \leftarrow \F^{k-1}$}. Prepare
        \begin{equation*}
            \frac{1}{\sqrt{|A|}}\sum_{v_0 \in A}\ket{v_0}_{C_1} \otimes 
            \ket{S_{u+v_0,w}}_{A_1},\, b\|\ell_{A_2},
        \end{equation*}
        where $A = \co(S) \cap T$.
        \item \textcolor{red}{Apply the isometry $\Is:\ket{v_0}_{C_1}\ket{0}_{C_2} \mapsto \ket{v_0}_{C_1}\Ket{\regR_{-1}\regB^{-1}(v_0+u)}_{C_2}$}
        \item Measure $C_2$ in computational basis and obtain $\ell' \in \F^{k-1}$.
        \item Initialize $\As_\lambda$ with
        $A_1A_2$ and $\Zs(S, T, u, w, 0^k)$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$.
        \item Apply $U$ on register $C_1$. Measure $C_1$ and obtain $\widetilde{v}_0$. Parse $\widetilde{v}_0 := \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in \left(S^+\right)^\perp / T^\perp$.
        \item If $\widetilde{z} \not\in S^\perp + w$ or $\widetilde{z} \in \left(S^+\right)^\perp + \widetilde{v}_{0c}+w$, then return $I-\cM$. Otherwise, output $\cM$.
    \end{enumerate}

    \paragraph{$\hyb_3^d$:} In this hybrid, some operations acting on different registers are reordered.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and a leakage $\ell \leftarrow \F^{k-1}$. Prepare
        \begin{equation*}
            \frac{1}{\sqrt{|A|}} \sum_{v_0 \in A}\ket{v_0}_{C_1} \otimes 
            \ket{S_{u+v_0,w}}_{A_1},\, b\|\ell_{A_2},
        \end{equation*}
        where $A = \co(S) \cap T$.
        \item Apply the isometry $\Is:\ket{v_0}_{C_1}\ket{0}_{C_2} \mapsto \ket{v_0}_{C_1}\Ket{\regR_{-1}\regB^{-1}(v_0+u)}_{C_2}$
        \item \textcolor{red}{Apply $U$ on register $C_1$. Measure $C_1$ and obtain $\widetilde{v}_0$. Parse $\widetilde{v}_0 := \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in \left(S^+\right)^\perp / T^\perp$.}
        \item Measure $C_2$ in computational basis and obtain $\ell'$.
        \item Initialize $\As_\lambda$ with
        $A_1A_2$ and $\Zs(S, T, u, w, 0^k)$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$.
        \item If $\widetilde{z} \not\in S^\perp + w$ or $\widetilde{z} \in \left(S^+\right)^\perp + \widetilde{v}_{0c}+w$, then return $I-\cM$. Otherwise, output $\cM$.
    \end{enumerate}

    \paragraph{$\hyb_3^e$:} In this hybrid, Step 1 of $\hyb_3^e$ computes the result of Steps 1 through 4 of $\hyb_3^d$.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and a leakage $\ell \leftarrow \F^{k-1}$. \textcolor{red}{Prepare}
        \begin{equation*}
            \sqrt{\frac{|\F|^{k-1}}{|A|\cdot |S|}}  \ \sum_{\substack{s \in S^+ \\ z:=s+g(s,u,\ell')+u}} \omega_{|\F|}^{z \cdot (\widetilde{v}_0+w)}  \ket{z}_{A_1},\, b\|\ell_{A_2},
        \end{equation*}
        for a uniformly random $\widetilde{v}_{0} \leftarrow B:= \co(T^\perp) \cap S^\perp$ and $\ell' \leftarrow \F^{k-1}$. Let $\widetilde{v}_{0} = \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in \left(S^+\right)^\perp / T^\perp$. Also, $g$ is defined as follows:
        Given $s:=s'+v_{0c}$ with $s' \in S$ and $v_{0c} \in A$, as well as $u \in \co(T)$. By the Row-Resilient Column Independence properties,
        there exists a unique vector, defined as 
        \begin{equation*}
            g(s,u,\ell') \in T/S^+
        \end{equation*}
        such that if $v_0:=v_{0c}+g(s,u,\ell') \in A$, then
        \begin{equation*}
            \regR_{-1}\regB^{-1}(v_0+u) = \ell'.
        \end{equation*}
        
        \item Initialize $\As_\lambda$ with
        $A_1A_2$ and $\Zs(S, T, u, w, 0^k)$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$.
        \item If $\widetilde{z} \not\in S^\perp + w$ or $\widetilde{z} \in \left(S^+\right)^\perp + \widetilde{v}_{0c}+w$, then return $I-\cM$. Otherwise, output $\cM$.
    \end{enumerate}

    \paragraph{$\hyb_3^f$:} In this hybrid, $\Zs(S, T, u, w, 0^k)$ is replaced by a simulator $\cS(G, T, u, x, 0^k)$.
    \begin{enumerate}
        \item Sample $[S,T]$ uniformly at random over $\F^n$ with $k$-dimensional leakage. Sample vectors $(u,w) \leftarrow \co(T) \times \co(S^\perp)$, a field $b \leftarrow \F$, and a leakage $\ell \leftarrow \F^{k-1}$. Prepare
        \begin{equation*}
            \sqrt{\frac{|\F|^{k-1}}{|A|\cdot |S|}}  \ \sum_{\substack{s \in S^+ \\ z:=s+g(s,u,\ell')+u}} \omega_{|\F|}^{z \cdot (\widetilde{v}_0+w)}  \ket{z}_{A_1},\, b\|\ell_{A_2},
        \end{equation*}
        for a uniformly random $\widetilde{v}_{0} \leftarrow B:= \co(T^\perp) \cap S^\perp$ and $\ell' \leftarrow \F^{k-1}$. Let $\widetilde{v}_{0} = \widetilde{v}_{0c} + \widetilde{v}_{0d}$, where $\widetilde{v}_{0c} \in S^\perp / \left(S^+\right)^\perp$ and $\widetilde{v}_{0d} \in  \left(S^+\right)^\perp / T^\perp$. Sample a subspace $G$ uniformly at random such that $S^\perp \leq G$, and $\dim(G) = \frac{3n}{4}$. Let $x \in \co(G)$ be the unique coset such that $S^\perp + w \subset G + x$. 
        
        \item Initialize $\As_\lambda$ with
        $A_1A_2$ and $\textcolor{red}{\cS(G, T, u, x, 0^k)}$. $\As_\lambda$'s output is parsed as a string $\widetilde{z} \in \F^{n}$.
        \item If $\widetilde{z} \not\in S^\perp + w$ or $\widetilde{z} \in \left(S^+\right)^\perp + \widetilde{v}_{0c}+w$, then return $I-\cM$. Otherwise, output $\cM$.
    \end{enumerate}




\begin{lemma}\label[lemma]{coset_ab}
    For all $m \in \F^k$, $\Pr\Big[\hyb_3^a(m)=I-\Ms \Big]  \geq \Pr\Big[\hyb_3^b(m)=I-\Ms\Big] - \negl(\lambda)$.
\end{lemma}
\begin{proof}
    In $\hyb_3^b$, we measure the $C_2$ register before sending the quantum state to the adversary. Since the adversary operates on different registers, their operation commutes with the measurement on $C_2$.

    Next, suppose (by contradiction) that there exists a polynomial $p(\cdot)$ such that for infinite many $\lambda$, $\Pr\Big[\hyb_3^a(m) = I-\cM\Big] < \Pr\Big[\hyb_3^b(m) = I-\cM\Big] - \frac{1}{p(\lambda)}$. We will construct a reduction $\cR$ that breaks the security of subspace-hiding. The reduction $\cR$ runs exactly as the experiment $\hyb_3^b$, except that in Step 3, $\As_{\lambda}$'s registers are initialized as $A_1A_2, ch$, where $ch$ is either $\cZ(S,T,u,w,r)$ or $\cZ(S,T,u,w,0^k)$, as sent by the challenger. By \cref{coset_stateconstruct,coset_unitaryconstruct}, all operations except the adversary can be implemented efficiently (This is why we say the predicate is efficiently checkable), and hence $\cR \in \mathscr{A}$. Finally, if the experiment outputs $\cM$, $\cR$ output $c_a'= 0$, i.e., $\cR$ guesses the challenge is $\cZ(S,T,u,w,r)$. Otherwise, $\cR$ outputs $c_a'= 1$. Then, $\cR$ breaks the security of subspace-hiding with advantage $\frac{1}{2\cdot p(\lambda)}$.
\end{proof}
    
\begin{lemma}\label[lemma]{coset_bc}
    For all $m \in \F^k$, $\hyb_3^b(m)=\hyb_3^c$.
\end{lemma}
\begin{proof}
    The following first term is the state described in $\hyb_3^b(m)$ at Step~1.
%    \shota{Is the normalization factor right here? (Seems missing sqrt)}
    \begin{align}
        &\frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} \ \ket{v_0}_{C_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{C_2} \otimes \nonumber \\
        &\ket{S_{v_0+u,w}}_{A_1}\Ket{b\|(m+\regR \regB^{-1} (v_0+u)+r)[2:k]}_{A_2} \nonumber \\
        \xmapsto{\text{Measure } C_2} \  &\frac{1}{\sqrt{|A|}} \sum_{\substack{v_0 \in A \\ (m+ \regR \regB^{-1}(v_0+u)+r)[2:k]=\ell}} \ \ket{v_0}_{C_1}\otimes 
        \ket{S_{v_0+u,w}}_{A_1},\ b\|\ell_{C_2}, \ b\|\ell_{A_2} \nonumber \\
        = \ &\frac{1}{\sqrt{|A|}} \sum_{\substack{v_0 \in A \\ \regR_{-1} \regB^{-1}(v_0+u)=\ell-(m+r)[2:k]}} \ \ket{v_0}_{C_1}\otimes 
        \ket{S_{v_0+u,w}}_{A_1},\ b\|\ell_{C_2}, \ b\|\ell_{A_2} \label{coset_hyb3b}
    \end{align}
    By the Row-Resilient Column Independence properties, if we choose $v_0 \leftarrow A$ uniformly at random, then $\regR_{-1}\regB^{-1}(v_0)$ is uniformly distributed over $\F^{k-1}$. Hence, $\ell$ is uniformly sampled over $\F^{k-1}$ and independent to $r$.
    Hence, the state of $\hyb_3^b(m)$ after Step 2 is the mixed state of term~(\ref{coset_hyb3b}) over the randomness of $[S,T]$, $r$, $\ell$, $u$, $w$ and $b$, where they are sample uniformly and independent on their own domain. Next, we consider the mixed state of $\hyb_3^c$ after Step 3. The first term below corresponds to the state described in $\hyb_3^c$ at Step 1.
    %\shota{Is the normalization factor right here? (Seems missing sqrt)}
    \begin{align}
        &\frac{1}{\sqrt{|A|}} \sum_{v_0 \in A}\ket{v_0}_{C_1} \otimes 
        \ket{S_{u+v_0,w}}_{A_1},\ b\|\ell_{A_2} \nonumber \\
        \xmapsto{\cI} \ &\frac{1}{\sqrt{|A|}} \sum_{v_0 \in A}\ket{v_0}_{C_1}\Ket{\regR_{-1}\regB^{-1}(v_0+u)}_{C_2} \otimes 
        \ket{S_{u+v_0,w}}_{A_1},\ b\|\ell_{A_2} \nonumber \\
        \xmapsto{\text{Measure } C_2} \ &\frac{1}{\sqrt{|A|}} \sum_{\substack{v_0 \in A \\ \regR_{-1} \regB^{-1}(v_0+u)=\ell'}} \ \ket{v_0}_{C_1}\otimes 
        \ket{S_{v_0+u,w}}_{A_1},\ \ell'_{C_2}, \ b\|\ell_{A_2} \label{coset_hyb3c}
    \end{align}
    Again, by Row-Resilient Column Independence properties, $\ell'$ is uniformly sampled over $\F^{k-1}$ and trivially independent to $\ell$. Hence, the state of $\hyb_3^c(m)$ after Step 3 is the mixed state of term~(\ref{coset_hyb3c}) over the randomness of $[S,T]$, $\ell$, $\ell'$, $u$, $w$, and $b$, where they are sample uniformly and independent on their own domain.

    In $\hyb_3^b(m)$, it uses the view of registers $C_1A_1$, as well as variables $b\|\ell_{A_2}$, $\ell-(m+r)[2:k]$, $\Zs(S, T, u, w, 0^k)$, $[S,T]$, and $w$ to obtain output. Similarly, in $\hyb_3^c(m)$, it uses the view of registers $C_1A_1$, as well as variables $b\|\ell_{A_2}$, $\ell'$, $\Zs(S, T, u, w, 0^k)$, $[S,T]$, and $w$ to obtain output. It appears that the distribution of both hybrids' view is identical.
\end{proof}

\begin{lemma}\label[lemma]{coset_cd}
    $\hyb_3^c=\hyb_3^d$.
\end{lemma}
\begin{proof}
    The difference between the two hybrids is just the reordering of commutable operations, and hence their output distributions are identical.
\end{proof}


\begin{lemma}\label[lemma]{coset_applyU}
    $\hyb_3^d=\hyb_3^e$.
\end{lemma}
\begin{proof}
    The following first term is the state at Step 1 in $\hyb_3^d$.
%    \synote{Is the normalizatino factor of the first line $\frac{1}{\sqrt{|A|}}$?}
 
    % \begin{align*}
    %     &\frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} \ket{v_0} \otimes \ket{S_{v_0+u,w}} 
    %     \\
    %     \xmapsto{\text{Apply } \cI \text{ and } U} \quad&\frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} (U\ket{v_0}) \otimes \ket{S_{v_0+u,w}} \otimes  \Ket{\regR_{-1}\regB^{-1}(v_0+u)} 
    %     \\      
    %     = \quad& \frac{1}{\sqrt{|A|\cdot |S|}}  \sum_{v_0 \in A} \ \sum_{z \in S + v_0 + u} (U\ket{v_0}) \otimes \omega_{|\F|}^{z \cdot w}\ket{z} \otimes \Ket{\regR_{-1}\regB^{-1}(v_0+u)}_{C_2}
    %     \\      
    %     \xmapsto{\text{Measure } C_2 \text{ and obtain } \ell'} \quad& \sqrt{\frac{|\F|^{k-1}}{|A|\cdot |S|}}  \sum_{\substack{s' \in S,\ v_{0c} \in S^+/S \\ z:=s'+v_{0c}+g(s'+v_{0c},u,\ell')+u}} (U\ket{v_0}) \otimes \omega_{|\F|}^{z \cdot w}\ket{z}, \text{ where } v_0:=v_{0c}+g(s'+v_{0c},u,\ell') \in A
    %     \\
    %     = \quad& \sqrt{\frac{|\F|^{k-1}}{|A|^2\cdot |S|}}   \ \sum_{\widetilde{v}_0 \in B}\ \sum_{\substack{s' \in S,\ v_{0c} \in S^+/S \\ z:=s'+v_{0c}+g(s'+v_{0c},u,\ell')+u}} \omega_{|\F|}^{v_0 \cdot \widetilde{v}_0} \cdot \omega_{|\F|}^{z \cdot w} \ket{\widetilde{v}_0} \otimes \ket{z} 
    %     \\
    %     = \quad& \sqrt{\frac{|\F|^{k-1}}{|A|^2\cdot |S|}}  \ \sum_{\widetilde{v}_0 \in B}\ \sum_{\substack{s' \in S,\ v_{0c} \in S^+/S \\ z:=s'+v_{0c}+g(s'+v_{0c},u,\ell')+u}} \omega_{|\F|}^{z \cdot (\widetilde{v}_0+w)}  \ket{\widetilde{v}_0}_{C_1} \otimes \ket{z} 
    %     \\
    %     \xmapsto{\text{Measure } C_1} \quad& \sqrt{\frac{|\F|^{k-1}}{|A|\cdot |S|}}  \ \sum_{\substack{s \in S^+ \\ z:=s+g(s,u,\ell')+u}} \omega_{|\F|}^{z \cdot (\widetilde{v}_0+w)}  \ket{z}.
    % \end{align*}
\begin{align*}
&\frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} \ket{v_0} \otimes \ket{S_{v_0+u,w}}
\\
\xmapsto{\text{Apply } \cI \text{ and } U}\quad
&\frac{1}{\sqrt{|A|}} \sum_{v_0 \in A} (U\ket{v_0}) \otimes \ket{S_{v_0+u,w}}
   \otimes \Ket{\regR_{-1}\regB^{-1}(v_0+u)}
\\
= \quad
&\frac{1}{\sqrt{|A|\cdot |S|}} \sum_{v_0 \in A}\sum_{z \in S + v_0 + u}
   (U\ket{v_0}) \otimes \omega_{|\F|}^{z \cdot w}\ket{z}
\\
&\qquad\otimes \Ket{\regR_{-1}\regB^{-1}(v_0+u)}_{C_2}
\\
\xmapsto{\text{Measure } C_2 \text{ and obtain } \ell'}\quad
&\sqrt{\frac{|\F|^{k-1}}{|A|\cdot |S|}}
  \sum_{\substack{s' \in S \\ v_{0c} \in S^+/S}}
  (U\ket{v_0}) \otimes \omega_{|\F|}^{z \cdot w}\ket{z},
\intertext{where \quad
$z := s' + v_{0c} + g(s' + v_{0c},u,\ell') + u$
\quad and \quad
$v_0 := v_{0c} + g(s' + v_{0c},u,\ell') \in A$.}
= \quad
&\sqrt{\frac{|\F|^{k-1}}{|A|^2\cdot |S|}}
  \sum_{\widetilde{v}_0 \in B}\ \sum_{\substack{s' \in S \\ v_{0c} \in S^+/S}}
  \omega_{|\F|}^{v_0 \cdot \widetilde{v}_0}\cdot \omega_{|\F|}^{z \cdot w}
  \ket{\widetilde{v}_0} \otimes \ket{z}
\\
= \quad
&\sqrt{\frac{|\F|^{k-1}}{|A|^2\cdot |S|}}
  \sum_{\widetilde{v}_0 \in B}\ \sum_{\substack{s' \in S \\ v_{0c} \in S^+/S}}
  \omega_{|\F|}^{z \cdot (\widetilde{v}_0+w)}
  \ket{\widetilde{v}_0}_{C_1} \otimes \ket{z}
\\
\xmapsto{\text{Measure } C_1}\quad
&\sqrt{\frac{|\F|^{k-1}}{|A|\cdot |S|}}
  \sum_{s \in S^+} \omega_{|\F|}^{z \cdot (\widetilde{v}_0+w)} \ket{z},
\intertext{where \quad $z := s + g(s,u,\ell') + u$.}
\end{align*}


    After measuring $C_2$, suppose we obtain a result $\ell'$. By the Row-Resilient Column Independence properties, $\ell'$ is sampled uniformly over $\F^{k-1}$. Again, by the Row-Resilient Column Independence properties, given $s'+v_{0c} \in S^+$ and $u \in \co(T)$,
    there exists a unique vector, defined as 
    \begin{equation*}
        g(s'+v_{0c},u,\ell') \in T/S^+
    \end{equation*}
    such that if $v_0:=v_{0c}+g(s'+v_{0c},u,\ell') \in A$, then
    \begin{equation*}
        \regR_{-1}\regB^{-1}(v_0+u) = \ell'.
    \end{equation*}

    Next, we show that the last equality holds, by showing that $z \cdot \widetilde{v}_0 = v_0\cdot \widetilde{v}_0$. Indeed, 
    \begin{equation*}
        z \cdot \widetilde{v}_0 = \left(s'+v_{0c}+ g(s',u,\ell')+u\right) \cdot \widetilde{v}_0 = (v_{0c}+ g(s,u,\ell')) \cdot \widetilde{v}_0 =  v_0\cdot \widetilde{v}_0
    \end{equation*}
    The second equality follows from the fact that $\widetilde{v}_0 \in \co(T^\perp) \cap S^\perp$, $s' \in S$, and $u \in \co(T)$.
    
    Finally, $\widetilde{v}_{0}$ in the last term is uniformly sampled over $B:=\co(T^\perp) \cap S^\perp$. It turns out that the final state is the state at Step 1 in $\hyb_3^e$.
\end{proof}

\begin{lemma}\label[lemma]{coset_ef}
    $\left|\Pr\Big[\hyb_3^e\Big]-\Pr\Big[\hyb_3^f\Big]\right| \leq \negl(\lambda)$.
\end{lemma}
\begin{proof}
    This follows from the subspace hiding property and from the fact that the experiment can be implemented within the class $\mathscr{A}$. The proof is similar to \cref{coset_ab}.
\end{proof}

\begin{lemma}\label[lemma]{coset_f}
    $\Pr\left[\hyb_3^f = I-\cM\right] = 1-\negl(\lambda)$.
\end{lemma}
\begin{proof}
    The adversary's view is completely determined by $(G,S^+,T, u,\widetilde{v}_{0c}+\widetilde{v}_{0d}+w, x, b\|\ell, \ell')$. For the rest of the proof, fix any valid choice of these variables. Given those variables, $\widetilde{z}$ is independent of $S^\perp + w $, where $S^\perp+w$ is a uniformly random subspace coset such that $\dim(S^\perp) = \frac{n}{2}$, $\left(S^+ \right)^\perp \leq S^\perp \leq G$, and $\left(S^+\right)^\perp + \widetilde{v}_{0c} + w  \leq S^\perp + w \leq G+x$. Indeed, $b\|\ell$ is sampled independentlly to any other variables. Also, $u$ and $\ell'$ have nothing to do with $S$ and $w$. Finally, $T^\perp \subset \left(S^+\right)^\perp$ also implies that $T$ is independent to the random choice of $S^\perp + w$. Then, we have 
    %\footnote{Most of the calculation is the same as in Claim 6.6 of \cite{BGK+}. However, their third equality, which corresponds to our third equality, contains a minor inaccuracy. The quantity they compute is a random subset containing $T^\perp + \widetilde{v}$, whereas it should be a random subspace. Nonetheless, the resulting bound remains correct asymptotically.} 
    \begin{align*}
        &\Pr\left[\hyb_3^f(m) = \cM\right] \\
        = &\Pr_{S,w}\left[ \widetilde{z} \in \left( S^\perp+w \right) \Big\backslash \left( (S^+)^\perp + \widetilde{v}_{0c} + w \right) \right] \\
        \leq  &\max_{z \in \F^n} \Pr_{S,w}\left[ z \in \left( S^\perp+w \right) \Big\backslash \left( (S^+)^\perp + \widetilde{v}_{0c} + w \right) \right] \\
        =  &\max_{z \in (G+x) \big\backslash \left( (S^+)^\perp + \widetilde{v}_{0c} + w \right)  } \Pr_{S,w}\left[ z \in \left( S^\perp+w \right)  \right] \\
        = & \frac{|\F|^{\dim S^\perp-\dim (S^+)^\perp}-1}{|\F|^{\dim G-\dim (S^+)^\perp}-1} \\
        = &\frac{|\F|^{n/4-k+1}-1}{|\F|^{n/2-k+1}-1} \\
        %=& \frac{|S^\perp + w| - \left|(S^+)^\perp + \widetilde{v}_{0c} + w\right|}{|G+x|- \left|(S^+)^\perp + \widetilde{v}_{0c} + w\right|} \\
        %=& \frac{2^{\frac{n}{2}} - 2^{\frac{n}{4}+k-1} }{2^{\frac{3n}{4}} - 2^{\frac{n}{4}+k-1} } \\
        =& \negl(\lambda).
    \end{align*}
\end{proof}
\end{proof}

